Diffusion Models with Anisotropic Gaussian Splatting for Image Inpainting

Image inpainting is a fundamental task in computer vision, aiming to restore missing or corrupted regions in images realistically. While recent deep learning approaches have significantly advanced the state-of-the-art, challenges remain in maintaining structural continuity and generating coherent textures, particularly in large missing areas. Diffusion models have shown promise in generating high-fidelity images but often lack the structural guidance necessary for realistic inpainting. We propose a novel inpainting method that combines diffusion models with anisotropic Gaussian splatting to capture both local structures and global context effectively. By modeling missing regions using anisotropic Gaussian functions that adapt to local image gradients, our approach provides structural guidance to the diffusion-based inpainting network. The Gaussian splat maps are integrated into the diffusion process, enhancing the model's ability to generate high-fidelity and structurally coherent inpainting results. Extensive experiments demonstrate that our method outperforms state-of-the-art techniques, producing visually plausible results with enhanced structural integrity and texture realism.

==> files/temp.tex <==
\section{Methods}

In this section, we present a method for image inpainting and restoration using Gaussian splatting. The method introduces anisotropic Gaussian modeling, multi-scale integration, and advanced network architectures incorporating attention mechanisms. The proposed method consists of three main components: enhanced Gaussian splatting of missing regions, a multi-scale generative inpainting network guided by the Gaussian models, and loss functions for training.

\subsection{Enhanced Gaussian Splat Modeling of Missing Regions}

\subsubsection{Anisotropic Gaussian Functions for Spatial Influence}

To capture the uncertainty and spatial influence around missing regions, we model each missing pixel using anisotropic Gaussian functions that adapt to local image structures. For each pixel location $ (x, y) $ in the missing region ($ M(x, y) = 1 $), we define a 2D anisotropic Gaussian function $ G_{x,y} $ as:

\begin{equation}
G_{x,y}(u, v) = \exp\left( -\frac{1}{2} 
\begin{bmatrix}
u - x & v - y
\end{bmatrix}
\Sigma_{x,y}^{-1}
\begin{bmatrix}
u - x \\ v - y
\end{bmatrix}
\right)
\end{equation}

where $ (u, v) $ are spatial coordinates in the image domain, and $ \Sigma_{x,y} $ is the covariance matrix at pixel $ (x, y) $, capturing the local structure and directionality~\cite{perona1990scale}.

\subsubsection{Covariance Matrix Estimation}

We estimate the covariance matrix $ \Sigma_{x,y} $ based on the local gradient information from the edge map $ E $. Specifically, we compute the gradient vectors $ \nabla E $ and estimate the structure tensor $ \mathbf{J}_{x,y} $:

\begin{equation}
\mathbf{J}_{x,y} = 
\sum_{(i,j) \in \mathcal{N}(x,y)}
\begin{bmatrix}
E_x(i,j) E_x(i,j) & E_x(i,j) E_y(i,j) \\
E_x(i,j) E_y(i,j) & E_y(i,j) E_y(i,j)
\end{bmatrix}
\end{equation}

where $ E_x $ and $ E_y $ are the gradients of $ E $ in the $ x $ and $ y $ directions, and $ \mathcal{N}(x,y) $ is a local neighborhood around $ (x,y) $~\cite{canny1986computational}.

We then define the covariance matrix $ \Sigma_{x,y} $ as the inverse of the regularized structure tensor:

\begin{equation}
\Sigma_{x,y} = \left( \mathbf{J}_{x,y} + \epsilon \mathbf{I} \right)^{-1}
\end{equation}

where $ \epsilon $ is a small positive constant to prevent singularity, and $ \mathbf{I} $ is the identity matrix.

\subsubsection{Adaptive Amplitude Modulation}

To account for the varying influence of each Gaussian splat, we assign an amplitude $ A_{x,y} $ based on the distance to the known regions:

\begin{equation}
A_{x,y} = \exp\left( -\beta d_{x,y} \right)
\end{equation}

where $ d_{x,y} $ is the distance to the nearest known pixel, computed as:

\begin{equation}
d_{x,y} = \min_{(i,j) \in \mathcal{K}} \sqrt{(x - i)^2 + (y - j)^2}
\end{equation}

and $ \beta $ is a scaling factor controlling the rate of decay, and $ \mathcal{K} = \{ (i, j) \mid M(i, j) = 0 \} $.

\subsubsection{Generation of Gaussian Splat Map}

For the entire missing region, we aggregate the anisotropic Gaussian functions weighted by their amplitudes to form the Gaussian splat map $ S $:

\begin{equation}
S(u, v) = \sum_{(x, y) \in \mathcal{M}} A_{x,y} \, G_{x,y}(u, v)
\end{equation}

where $ \mathcal{M} = \{ (x, y) \mid M(x, y) = 1 \} $.

\subsubsection{Normalization and Multi-Scale Integration}

To capture information at different scales, we compute the Gaussian splat maps at multiple scales by varying the neighborhood size in covariance estimation~\cite{lindeberg1994scale}. The final splat map $ S_{\text{norm}} $ is obtained by normalizing and combining the multi-scale splat maps:

\begin{equation}
S_{\text{norm}}(u, v) = \frac{S(u, v) - S_{\text{min}}}{S_{\text{max}} - S_{\text{min}}}
\end{equation}

where $ S_{\text{min}} $ and $ S_{\text{max}} $ are the minimum and maximum values of $ S $ across all scales.

\subsection{Multi-Scale Generative Inpainting Network with Attention}

\subsubsection{Network Architecture}

We design a multi-scale generative inpainting network that incorporates attention mechanisms to effectively utilize the Gaussian splat guidance. The network consists of several scales, each containing encoder-decoder layers with skip connections across scales to facilitate information flow~\cite{ronneberger2015u}.

\subsubsection{Attention Mechanisms}

We integrate spatial attention modules that use the Gaussian splat map to focus the network's attention on regions with higher uncertainty~\cite{wang2018non, zhang2019self}. The attention map $ A_{\text{att}} $ is computed as:

\begin{equation}
A_{\text{att}} = \sigma\left( \text{Conv}(S_{\text{norm}}) \right)
\end{equation}

where $ \text{Conv} $ represents convolutional layers and $ \sigma $ is the sigmoid activation function.

\subsubsection{Input to the Network}

The input to the network $ \mathcal{N} $ at each scale is a concatenation of the incomplete image, the mask, the Gaussian splat map, the edge map, and the attention map:

\begin{equation}
X = \left[ (I \odot (1 - M)),\ M,\ S_{\text{norm}},\ E,\ A_{\text{att}} \right]
\end{equation}

\subsubsection{Loss Functions}

To train the network, we employ a combination of loss functions that encourage the generation of realistic and coherent content.

\paragraph{Reconstruction Loss ($ \mathcal{L}_{\text{rec}} $):}

\begin{equation}
\mathcal{L}_{\text{rec}} = \| (\hat{I} - I) \odot (1 - M) \|_1
\end{equation}

\paragraph{Perceptual Loss ($ \mathcal{L}_{\text{perc}} $):}

\begin{equation}
\mathcal{L}_{\text{perc}} = \sum_{l} \| \phi_l(\hat{I}) - \phi_l(I) \|_2^2
\end{equation}

where $ \phi_l $ represents the activation maps from layer $ l $ of a pretrained VGG-19 network~\cite{simonyan2014very}.

\paragraph{Style Loss ($ \mathcal{L}_{\text{style}} $):}

\begin{equation}
\mathcal{L}_{\text{style}} = \sum_{l} \| \mathcal{G} \left( \phi_l(\hat{I}) \right) - \mathcal{G} \left( \phi_l(I) \right) \|_1
\end{equation}

where $ \mathcal{G}(\cdot) $ computes the Gram matrix of the feature maps~\cite{gatys2016image}.

\paragraph{Total Variation Loss ($ \mathcal{L}_{\text{tv}} $):}

\begin{equation}
\mathcal{L}_{\text{tv}} = \sum_{i,j} \left( (\hat{I}_{i+1,j} - \hat{I}_{i,j})^2 + (\hat{I}_{i,j+1} - \hat{I}_{i,j})^2 \right)
\end{equation}

\paragraph{Adversarial Loss ($ \mathcal{L}_{\text{adv}} $):}

We employ a PatchGAN discriminator $ D $ to enforce local realism~\cite{isola2017image}:

\begin{equation}
\begin{split}
\mathcal{L}_{D} &= - \mathbb{E}_{I} [\log D(I)] - \mathbb{E}_{\hat{I}} [\log (1 - D(\hat{I}))] \\
\mathcal{L}_{\text{adv}} &= - \mathbb{E}_{\hat{I}} [\log D(\hat{I})]
\end{split}
\end{equation}

\paragraph{Total Loss:}

The total loss function is a weighted sum of the individual losses:

\begin{equation}
\mathcal{L}_{\text{total}} = \lambda_{\text{rec}} \mathcal{L}_{\text{rec}} + \lambda_{\text{perc}} \mathcal{L}_{\text{perc}} + \lambda_{\text{style}} \mathcal{L}_{\text{style}} + \lambda_{\text{tv}} \mathcal{L}_{\text{tv}} + \lambda_{\text{adv}} \mathcal{L}_{\text{adv}}
\end{equation}

where $ \lambda_{\text{rec}} $, $ \lambda_{\text{perc}} $, $ \lambda_{\text{style}} $, $ \lambda_{\text{tv}} $, and $ \lambda_{\text{adv}} $ are hyperparameters.

\subsubsection{Network Training}

We adopt a progressive training strategy, training the network scale by scale, starting from the coarsest scale to the finest, allowing for better convergence and performance~\cite{karras2017progressive}.

\paragraph{Stage-wise Training}

In each stage, we train the network components corresponding to that scale while keeping the parameters of the other scales fixed.

\subsection{Implementation Details}

\subsubsection{Hyperparameters}

\begin{itemize}
    \item \textbf{Covariance Regularization Constant} ($ \epsilon $): Typically set to $ 1 \times 10^{-5} $.
    \item \textbf{Amplitude Decay Factor} ($ \beta $): Set empirically, e.g., $ \beta = 0.1 $.
    \item \textbf{Loss Weights}:
    \begin{itemize}
        \item $ \lambda_{\text{rec}} = 1.0 $
        \item $ \lambda_{\text{perc}} = 0.1 $
        \item $ \lambda_{\text{style}} = 250 $
        \item $ \lambda_{\text{tv}} = 0.1 $
        \item $ \lambda_{\text{adv}} = 0.01 $
    \end{itemize}
\end{itemize}

\subsubsection{Training Parameters}

\begin{itemize}
    \item \textbf{Optimizer}: Adam with $ \beta_1 = 0.5 $, $ \beta_2 = 0.999 $~\cite{kingma2014adam}.
    \item \textbf{Learning Rate}: $ 2 \times 10^{-4} $ for both generator and discriminator.
    \item \textbf{Batch Size}: 8.
    \item \textbf{Number of Epochs}: 50 per scale in the multi-scale training.
\end{itemize}

\subsubsection{Data Augmentation}

We apply data augmentation techniques during training, including random scaling, rotation, and flipping, to improve the robustness of the model~\cite{shorten2019survey}.

\subsection{Evaluation Metrics}

To assess the performance of the proposed method, we use the following quantitative metrics:

\begin{itemize}
    \item \textbf{Peak Signal-to-Noise Ratio (PSNR)}: Measures the similarity between the inpainted image and the ground truth~\cite{hore2010image}.
    \item \textbf{Structural Similarity Index (SSIM)}: Evaluates the perceived quality of the inpainted image~\cite{wang2004image}.
    \item \textbf{MSE}: Mean-Squared Error.
\end{itemize}

Additionally, we perform qualitative evaluations by visual inspection of the inpainted results, focusing on the continuity of structures and the absence of artifacts.

\subsection{Comparative Experiments}

We compare our method with state-of-the-art inpainting algorithms. The methods compared include:

\begin{itemize}
    \item \textbf{Contextual Attention Network}~\cite{yu2018generative}
    \item \textbf{EdgeConnect}~\cite{nazeri2019edgeconnect}
    \item \textbf{Partial Convolutional Network}~\cite{liu2018image}
\end{itemize}

We evaluate the performance both quantitatively and qualitatively, focusing on structural continuity and realistic texture generation.
